Efficient Manipulation of Bose-Einstein Condensates in a Double-Well Potential

We pose the problem of transferring a Bose-Einstein Condensate (BEC) from one side of a double-well potential to the other as an optimal control problem for determining the time-dependent form of the potential. We derive a reduced dynamical system using a Galerkin truncation onto a finite set of eigenfunctions and find that including three modes suffices to effectively control the full dynamics, described by the Gross-Pitaevskii model of BEC. The functional form of the control is reduced to finite dimensions by using another Galerkin-type method called the chopped random basis (CRAB) method, which is then optimized by a genetic algorithm called differential evolution (DE). Finally, we discuss the extent to which the reduction-based optimal control strategy can be refined by means of including more modes in the Galerkin reduction.

==> BEC Transfers (arXiv)/macros.tex <==
% !TEX useTabs% These three definitions use \DeclarePairedDelimiter from mathtools
% Use with a * to get \left and \right
%\DeclarePairedDelimiter{\set}{\{}{\}}
\DeclarePairedDelimiterX{\innerp}[2]{\langle}{\rangle}{#1,#2}
\renewcommand{\ip}[2]{\innerp*{#1}{#2}}
%\DeclarePairedDelimiterX{\PB}[2]{\{}{\}}{#1,#2} % Poisson brackets

\newcommand{\normp}[2]{{\norm{#1}}_{#2}}

% We define a transpose command so we can code meaning not typesetting
% \newcommand{\transpose[1]{ {#1}^{\mathsf{T}} }}



% Shortcuts for some matrices, which are bold uppercase latin letters
\newcommand{\J}{\vb{J}}
\newcommand{\I}{\vb{I}}
\newcommand{\A}{\vb{A}}

% Shortcuts for some vectors, which are bold lowercase latin letters
\newcommand{\x}{\vb{x}}
\newcommand{\y}{\vb{y}}
\newcommand{\vw}{\vb{w}}

% There is already a command \r, so we have to use \renewcommand instead of \newcommand
\renewcommand{\r}{\vb{r}}
\newcommand{\Matlab}{\textsc{Matlab}}


\newcommand{\Md}{M_{\rm d}}
\newcommand{\psid}{\psi_{\rm d}}

% If you're using these often, you should make macros!
\newcommand{\CC}{{\mathbb C}}
\newcommand{\RR}{{\mathbb R}}
\newcommand{\ZZ}{{\mathbb Z}}

\newcommand{\footremember}[2]{%
    \footnote{#2}
    \newcounter{#1}
    \setcounter{#1}{\value{footnote}}%
}
\newcommand{\footrecall}[1]{%
    \footnotemark[\value{#1}]%
} 

% \makeatletter
% \renewcommand{\email}[2][]{%
%   \ifx\emails\@empty\relax\else{\g@addto@macro\emails{,\space}}\fi%
%   \@ifnotempty{#1}{\g@addto@macro\emails{\textrm{(#1)}\space}}%
%   \g@addto@macro\emails{#2}%
% }
% \makeatother

% \tracingmacros=1

==> BEC Transfers (arXiv)/packages.tex <==
% Packages I always call

% BiBTeX helper package that sorts citations and compresses consecutive numbered citations
\usepackage{tabularx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{boxedminipage}
\usepackage{appendix}
\usepackage{algorithm2e}
%\usepackage[Algorithm]{algorithm2e}
\RestyleAlgo{boxruled}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{subfigure}
% \usepackage{authblk}
% \usepackage[foot]{amsaddr}

%\usepackage[numbers,sort&compress]{natbib}  
\usepackage{cite}

% Package to allow for the inclusion of graphics files
\usepackage{graphicx}
\usepackage[export]{adjustbox}

% The breqn package allows \left and \right delimiters to match across line breaks. 
% It requires the flexisym package
\usepackage{flexisym}	 
\usepackage{breqn}       

% Several important packages for math and physics typesetting
\usepackage{amsmath,amssymb,amsthm}
\usepackage{mathtools}   % Some improvements to AMS-LaTeX
\usepackage{physics}

%%% Fix some problems due to TeX being a super-old program

% The inputenc package allows you for the direct input of diacritic characters
\usepackage[utf8]{inputenc} 

% These 2 lines automatically replace ordinary quotation marks
% with asymmetric opening and closing quotation marks
\usepackage{csquotes}     
\MakeOuterQuote{"}       

%%% Useful things for while you're writing. Disable for final submission.

% Package to eliminate whitespace so you can see as much of your text as possible
\usepackage{fullpage}

% Package to insert todo notes and to insert placeholders for missing figures
\usepackage[colorinlistoftodos]{todonotes}   

% Package to display labels, useful for remembering how you labeled things
%\usepackage{showlabels}  

\usepackage{hyperref} % adds hyper links inside the generated pdf file
 \hypersetup{%
 	colorlinks=true,       % false: boxed links; true: colored links
 	linkcolor=blue,          % color of internal links
 	citecolor=blue,        % color of links to bibliography
 	filecolor=magenta,      % color of file links
 	urlcolor=blue         
 }
%%%
